Beyond Worst-case Analysis of Multicore Caching Strategies

Every processor with multiple cores sharing a cache needs to implement a cache-replacement algorithm. Previous work demonstrated that the competitive ratio of a large class of online algorithms, including Least-Recently-Used (LRU), grows with the length of the input. Furthermore, even offline algorithms like Furthest-In-Future, the optimal algorithm in single-core caching, cannot compete in the multicore setting. These negative results motivate a more in-depth comparison of multicore caching algorithms via alternative analysis measures. Specifically, the power of the adversary to adapt to online algorithms suggests the need for a direct comparison of online algorithms to each other. In this paper, we introduce cyclic analysis, a generalization of bijective analysis introduced by Angelopoulos and Schweitzer [JACM'13]. Cyclic analysis captures the advantages of bijective analysis while offering flexibility that makes it more useful for comparing algorithms for a variety online problems. In particular, we take the first steps beyond worst-case analysis for analysis of multicore caching algorithms. We use cyclic analysis to establish relationships between multicore caching algorithms, including the advantage of LRU over all other multicore caching algorithms in the presence of locality of reference.

==> abstract.tex <==
\begin{abstract} % \small\baselineskip=9pt
  Every processor with multiple cores sharing a cache needs to implement a
    cache-replacement algorithm.   Previous work demonstrated that the
    competitive ratio of a large class of online algorithms, including
    Least-Recently-Used (LRU), grows with the length of the input. Furthermore,
    even offline algorithms like Furthest-In-Future, the optimal algorithm in
    single-core \paging, cannot compete in the \mc setting.  These negative
    results motivate a more in-depth comparison of \mc caching algorithms via
    alternative analysis measures. Specifically, the power of the adversary to
    adapt to online algorithms suggests the need for a direct comparison of
    online algorithms to each other.

  In this paper, we introduce cyclic analysis, a generalization of bijective
    analysis introduced by Angelopoulos and Schweitzer [JACM'13]. Cyclic
    analysis captures the advantages of bijective analysis while offering
    flexibility that makes it more useful for comparing algorithms for a
    variety online problems. In particular, we take the first steps beyond
    worst-case analysis for analysis of \mcp algorithms.  We use cyclic
    analysis to establish relationships between \mcp algorithms, including the
    advantage of LRU over all other \mc caching algorithms in the presence of
    locality of reference.
\end{abstract}

%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "main.tex"
%%%% End:


==> app-bijective-prelims.tex <==
\section{Definitions for~\secref{surjective}}\label{app:surjective-prelims}

In this appendix we formalize the high-level definitions and lemmas
from~\secref{surjective}.

\subheading{Schedule definitions}


\helen{moved definition of schedule to prelims. maybe we need to say something
  like ``recall definition of schedule from~\secref{prelim}}.

Let \req be a request sequence, \ma be a paging algorithm, and $n_{\req, \ma}$
be the time required for \ma to serve \req. Given an integer
$j \leq n_{\req, \ma}$, let
$\skedpre = \{\sked_{\req_1, \ma}[1, j], \ldots, \sked_{\req_p, \ma}[1, j]\},
\skedar[j+1] = (\sked_{\req_1, \ma}[j+1], \ldots,\sked_{\req_p, \ma}[j+1]),
\skedsuf =\{\sked_{\req_1, \ma}[j+2, m^\ma_1], \ldots, \sked_{\req_p, \ma}[j+2,
m^\ma_p]\}$ (where $m^\ma_i$ is how long (in time) it takes to serve $\req_i$
under \ma). Note that \skedpre or \skedsuf may be empty. Informally, $\skedpre$
is all the requests served up to time $j$ with repetitions matching scheduling
delay (prefix), $\skedar[j+1]$ is all requests served at time $j+1$, and
\skedsuf is all requests served after time $j+1$ with repetitions matching
scheduling delay (suffix).

Let $\req^{\leq t, \ma}$ be all subsequences from \req served up to time $t$ and
$\req^{> t, \ma}$ be all subsequences from \req served after time $t$. Also let
$r_t$ be the requests at time $t$. For simplicity, let
$\reqpre = \req^{\leq j, \ma}$ ( all subsequences from \req served up to time
$j$) and $ \reqsuf = \req^{> j+1, \ma}$ (all subsequences from \req served after
time $j+1$) when $j, \ma$ are understood from context.

Let \reqpre be all subsequences from \req served up to time $j$ and \reqsuf be
all subsequences from \req served after time $j+1$ (created by removing
repetitions due to scheduling delay from \skedpre, \skedsuf). Also let $r_{j+1}$
be the requests at time $j+1$.


Using the \lru example in~\figref{example-serve} when $j = 4$,
$\reqpre_1 = \sigma_1\sigma_2$, $\reqpre_2 = \sigma_3, \sigma_4$ because those
are the pages that have been requested until time $4$. Since at timestep $5$ all
processors are fetching requests, $r_{j+1} = \emptyset$. Also,
$\reqsuf_1 = \sigma_1\sigma_5$ and $\reqsuf_2 = \sigma_5\sigma_2$ because those
are the requests remaining after timestep $5$.  Similarly,
$\sked^{\text{pre}}_{\req_1} = \sigma_1\sigma_1\sigma_1\sigma_2$ and
$\sked^{\text{pre}}_{\req_2} = \sigma_3\sigma_3\sigma_3\sigma_4$. at timestep
$4$, both processors are fetching, so
$r^1_{j+1} = \sigma_2, r^2_{j+1} = \sigma_4$. The suffix is the schedule for
timesteps after $4$, so
$\sked^{\text{suf}}_{\req_1} = \sigma_2\sigma_1\sigma_5\sigma_5$ and
$\sked^{\text{suf}}_{\req_2} =\sigma_4\sigma_5\sigma_5\sigma_5\sigma_2$.


\subheading{\lru in the multi-core setting}

We formalize \defn{tag-based \lru}~\cite{AngeSc09} in a shared cache based on a
straightforward extension of the definition of tag-based \lru in the single-core
setting~\cite{AngeSc09}. \lru determines which page to evict depending on the
last timestamp each page was requested at. Index-based \lru may keep pages with
higher indices even if they were requested less-recently because some processor
may have ``run ahead'' of the other processors.

\begin{definition}[Tag-based Algorithm (adapted from~\cite{AngeSc09})]
  \label{def:tag-based}
  A \defn{tag-based} algorithm \ma assigns a set $T$ of (integer) \emph{tags} to
  each page in its cache. Formally, for every page $\sigma$ in \ma's cache, let
  $\text{tag}_\ma[\sigma, \skedar[t]]$ be the tag assigned to $\sigma$
  right after \ma has served requests up to timestep $t$. \ma is tag-based with
  respect to $T$ if it processes each request $\sigma$ at each timestep
  $\ell > t$ as follows:
  \begin{enumerate}
  \item If $\sigma$ is a hit, \mb updates the tag of $\sigma$ to $\ell$.
  \item If $\sigma$ is a fault and not currently being fetched by another
    processor, there are two cases. If the cache is full, \ma must evict a
    page. Otherwise, \ma may or may not evict a page. If \ma evicts a page, it
    will first evict from the cache the page of the smallest tag; then it will
    update the tag of page $\sigma$ to the current timestep to $\ell$ and
    continue updating it to $\ell + t'$ for the next $t' = 1, \ldots, \tau - 1$
    timesteps (that is, in each timestep $t + 1, \ldots, t + \tau$) until
    $\sigma$ has been fetched.
  \item If $\sigma$ is a fault and currently being fetched by another processor,
    let $x < \tau$ denote the remaining timesteps until $\sigma$ is brought to
    the cache. In this case, \ma will not evict a page (since the eviction due
    to $\sigma$ already happened) and stall for $x$ steps until $\sigma$ is
    brought to the cache.
  \end{enumerate}
\end{definition}

\defn{Tag-based \lru} is tag-based on \emph{all} timesteps while serving every
request sequence.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> app-cba.tex <==
\section{Proofs for~\secref{cba}}\label{app:cba}

\ccpcontra*

\begin{proof}
  If $\ma \bless \mb$, by~\defref{bij-analysis}, there must exist an \inp
  $\sigma \in \univ$ such that $\ma(\sigma) < \mb(\pi(\sigma))$. Let $\sigma$ be
  the \inp with the smallest cost that differs between $\ma, \mb$, and let
  $\univ^{\ma(\sigma)}_\ma, \univ^{\ma(\sigma)}_\mb \subset \univ$ be the
  sequences that have cost at most $\ma(\sigma)$ in $\ma(\univ), \mb(\univ)$,
  respectively. By the \ccp, $ |\univ^{\ma(\sigma)}_\ma|$ and
  $|\univ^{\ma(\sigma)}_\mb|$ are both bounded and
  $|\univ^{\ma(\sigma)}_\ma| > | \univ^{\ma(\sigma)}_\mb|$. It is impossible to
  define another function $\phi$ such that $\mb \bleq \ma$ because there are not
  enough \inps in $\univ^{\ma(\sigma)}_\mb$ to map to all \inps in
  $\univ^{\ma(\sigma)}_\ma$ such that the cost of each \inp under $\mb$ is at
  most the cost of the corresponding \inp under $\ma$.
\end{proof}

\unzipping*

\begin{proof}
  At a high level, we will describe how to convert a \surj surjective function
  $f$ into a bijective mapping $f_b$ by ``unzipping'' any many-to-one mappings
  in each partition. At a high level, the new mapping $f_b$  ``spaces'' in
  between each element in the sorted image.

  Let $X_m, Y_m$ be the pre-image and image of a non-empty mapping-based
  partition for any fixed $m \in \mathbb{N}$. Suppose we order the elements in
  $Y_m$ from lowest to highest and let $y_i$ be the $i$-th largest element in
  $Y_m$. Given an element $y_i \in Y_m$, let the corresponding elements in the
  pre-image be $x_{i, j} \in X_m$ for $j = 1, 2, \ldots, m$ in some
  order. Since $\ma(x_{i, j}) \leq \mb(y_i)$ for all $i, j$ (by the definition
  of surjective analysis), for any $i, j$, $\ma(x_{i, j}) \leq \mb(y_z)$ for
  $z > i$. Therefore, we define a new bijective mapping $f_b$ based on $f$ such
  that $f_b(x_{i, j}) = y_{mi + j - 1}$. The new mapping $f_b$ satisfies the
  property that for all $\sigma \in \univ$, $\ma(\sigma) \leq \mb(f_b(\sigma))$.
\end{proof}


==> app-figs.tex <==
% \section{Figures}\label{app:figs}

% \input{example-serve}

\begin{figure*}[t]
  \centering
  \includegraphics[width=12cm]{figs/lower-seq-redux-crop.pdf}
% \input{bigfi}
% \vspace*{2mm}
  \caption{An example of the alignment of \alg and \off described in
    ~\thmref{lower-shared-2} of two cores. For each sequence, easy \phases
    consist of cycles of requests to a two distinct pages (alternating short
    dark red and blue) combined with requests to a single page (light red and
    blue), while hard (long dark red and blue) \phases are adversarial and
    designed so \alg faults on every request.\newline \hspace{\textwidth} Left top:
    \alg serving all cores in their easy and hard \phases at the same
    time. \newline \hspace{\textwidth} Left bottom: Offline algorithm \off delaying
    \bluep. After the initial alignment, \off only faults at most $k$ times per
    core in each hard \phase and therefore needs at most $k$ faults in the easy
    \phases to maintain the alignment.\newline \hspace{\textwidth} Right: Examples of
    the cache state with $k = 10$ at each of the \tss marked $t_0, t_1,
    t_2$. At $t_0$, \alg has two red and two blue pages, while \off has one red
    and two blue pages. The yellow cells represent empty cells. At $t_1$, after
    the first red hard \phase, \alg also finishes its first blue hard \phase
    while \off finishes the first blue easy \phase. The light purple cells are
    those that could either be red or blue.  At \tss $t_2$ after \redp's first
    easy \phase, \alg has at least one of each color page in its cache, whereas
    \off might only have blue pages.}
 \label{fig:lower-shared}
\end{figure*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> app-noschedule.tex <==
\section{Proofs for~\secref{noschedule}}\label{app:nosked}

Before proving Theorem~\ref{thm:lru-no-schedule}, we prove the same result when $p=2$.

\begin{lemma}
  \label{thm:lru-no-schedule-two-cors}
  \slru is not competitive against an optimal offline algorithm \off with fetch
  time $\tau = 1$ when $p=2$.
\end{lemma}


\begin{proof}
  At a high level, we will define a sequence for two cores in phases such that
  \lru completes the first phase of each core at the same time, but \off
  finishes the first core's first phase early. \off generates an alignment so
  that it staggers the number of pages requested.~\figref{lru-no-schedule} shows
  the alignment of \lru versus \off.

  Suppose we have two cores $p_1, p_2$ and a request
  sequence $\sigma = (\req_1, \req_2)$ as follows:
  $$\req_1 = (\sigma_1, \ldots, \sigma_{k-1})^{\ell_1}[(\sigma^1_1, \ldots,
  \sigma^1_{k/2 + 1})^{\ell_3} (\sigma^1_a \sigma^1_b)^{\ell_4}]^\phi$$
  $$\req_2 = (\sigma_a, \sigma_b)^{\ell_2}[(\sigma^2_1, \ldots,
  \sigma^2_{k/2 + 1})^{\ell_3} (\sigma^2_a \sigma^2_b)^{\ell_4}]^\phi,$$ where
  $\ell_1, \ell_2, \ell_3, \ell_4$ are variables to be defined later.

  We call the first phase of $(\sigma_1, \ldots, \sigma_{k-1})^{\ell_1}$ and
  $(\sigma_a, \sigma_b)^{\ell_2}$ the introductory phase.  Let the request
  pattern of $(\sigma_1, \ldots, \sigma_{k/2 + 1})$ and $(\sigma_a, \sigma_b)$
  be a \defn{hard phase} and \defn{easy phase}, respectively.  The rest of the
  sequence after the introductory phase is defined by alternating hard and easy
  phases. We define the sequence such that for \lru, the hard phases of both
  cores are lined up, causing all faults in the hard phase, and such that
  \off lines up the easy phases with hard phases.

  We define $L$ as the time to complete the introductory phase for \lru. We want
  to construct the introductory phase so that both cores finish it at the same
  time, or $L = \ell_1(k-1)\tau = 2\tau + 2\ell_2$. Therefore,
  \begin{align*}
    \ell_1(k-1)\tau & = 2\tau + 2(\ell_2 - 1) \\
    \ell_2 & = \frac{\ell_1(k-1)\tau}{2} - \tau + 1
  \end{align*}

  We now want to define the remaining hard and easy phases based on the time
  left in the introductory phase for \off. The total number of requests in the
  introductory phase of $p_1$ and $p_2$ is $(k-1)\ell_1$ and $2\ell_2$,
  respectively. Let $L_{\text{rem}}$ be the number of requests remaining in the introductory
  phase of $p_2$ after finishing $p_1$ under \off.
  \begin{align*}
    L_{\text{rem}} & =  2\ell_2 - (k-1)\ell_1 \\
                    & = 2\left(\frac{\ell_1\tau(k-1)}{2} - \tau + 1\right)
                      - (k-1)\ell_1 \\
                    & = \ell_1\tau(k-1) - 2\tau + 2 - (k-1)\ell_1 \\
                    & = (\tau-1)(k-1)\ell_1 - 2\tau + 2 \\
                    & \approx (\tau-1)(k-1)\ell_1 \approx (\tau - 1)\ell_2
  \end{align*}

  We want to construct the sequence so that \off finishes its
  first hard phase in $p_1$ when $p_2$ finishes its introductory phase and to
  match the length of the easy phase and hard phase of \off.
  Therefore, the remaining lengths of hard and easy phases
  $\ell_3 = \frac{L_{\text{rem}}}{k/2 + 1}$ and
  $\ell_4 = \frac{ L_{\text{rem}}}{2}$, respectively.

  By construction, we repeat the easy and hard phases $\phi$ times each. Let
  $c_1$ be the number of requests in $\req_1$'s introductory phase, $c_2$ be the
  number of requests in $\req_2$'s introductory phase, $c_3$ be the number of
  requests in each hard phase, and $c_4$ be the number of requests in each easy
  phase.

  By construction, \lru faults on all requests in hard phases and all requests
  in the introductory phase of $\req_1$. \off faults only on the cold requests
  in each hard phase, and some of the requests in the introductory phase of
  $\req_1$

  The total number of requests for $p_1$ is $n_1 = c_1 + \phi(c_3 + c_4)$, the
  total number of requests for $p_2$ is $n_2 = c_2 + \phi(c_3 + c_4)$, and the
  total number of requests is $n = n_1 + n_2$.

  Let us set $c_1 = \sqrt{n_1}, \phi = \sqrt{n_1} - 1, c_3 + c_4 = \sqrt{n_1}$. By
  construction, $c_2 = O(kc_1)$, so $n_2 = O(kn_1)$. Also, the number of
  requests in the easy and hard phases $c_3, c_4$ are within an additive factor
  of $k\tau$. Therefore, the competitive ratio of \lru and \off is therefore as
  follows:

  \begin{align*}
    \frac{\lru(\sigma)}{\off(\sigma)} & \approx \frac{\phi c_3 + c_1}{\phi k + (c_1
                                            / k)} = \Omega(\sqrt{n}/k)
  \end{align*}
  Therefore, \lru is not competitive against \off.
\end{proof}


%\begin{Theor}
%  \lru is not competitive against an optimal offline algorithm \off with fetch
%  time $\tau = 1$ for any number of cores $p \geq 2$.
%\end{corollary}
% \lrunoschedule*

\begin{proof}
  We copy the request sequence but make the hard phase have $k/p + 1$ distinct
  requests instead of $k/2 + 1$ requests as in the proof
  of~\thmref{lru-no-schedule}. The lower bound will improve by a factor of $p$,
  which is dominated by the $\sqrt{n}$ term.
\end{proof}


\syncupper*

\begin{proof}
  We compare the cost of \aaa and \opt (with no schedule) on each phase.

  \pparagraph{Paging round:} At the beginning of each phase, both algorithms
  have seen the same number of requests (\aaa might be still fetching
  some). \aaa forces cores to be synced, and \opt has no schedule, so all cores
  are always synced. In the paging round, at most $k+j$ different pages are
  requested and the cost of \opt is at least $j$ where $1\leq j \leq p$. The
  extra factor of $j$ comes from the fact that at time-step $\hat{t}$, it is
  possible that $j$ new pages appear. The cost of \aaa is therefore at most
  $k+j$ in the paging round.

  \pparagraph{Scheduling round:} To count the number of faults in the scheduling
  rounds, we first bound how far any core might have lagged behind in the paging
  round. Let $f_i$ indicate the number of faults by core $p_i$ in the paging
  round ($\sum\limits_{i=1}^{p}f_i = k+j$). If core $p_i$ has $f_i$ faults and
  some $x_i$ number of hits in the paging round, the core that is the farthest
  ahead, $p^* \neq p_i$, had at most $x+f_i\tau$ hits in that round (for all
  $i$). Therefore, $p^*$ saw at most $f_i(\tau-1)$ more requests while $p_i$ was
  fetching.  In addition, the core $p_i$ could be fetching at the beginning
  of the round for at most $\tau-1$ time-steps, so $p^*$ would have seen at most
  $\tau-1$ pages while $p_i$ fetched.  Therefore, $p^*$ would have seen at most
  $(f_i+1) (\tau-1)$ more pages than $p_i$.

  Next, we bound the number of number of pages seen by each core in the
  scheduling rounds, which bounds the number of hits during the scheduling
  rounds.  Let $h_i$ denote the number of hits by $p_i$ during the $i$-th
  scheduling round and $X$ denote the length (in terms of the number of
  timesteps) of that round. The number of pages that $p_i$ sees during its
  scheduling round is at least $A=h_i + \lfloor (X-h_i)/\tau \rfloor$, while the
  number of pages $p^*$ sees is at most $B = \lceil X/\tau \rceil$ pages as it
  faults on every request. Since the two are synced at the end of the round, the
  difference between the number of pages they see should be at most the number
  of pages that $p^*$ saw more in the paging round. Therefore, the difference
  between the two cores $A-B \leq (f_i+1)(\tau-1)$ implies
  $h_i (1- 1/\tau) \leq (f_i+1)(\tau-1)$, which gives $h_i \leq (f_i+1)
  \tau$. Recall that $\sum\limits_{i=1}^{p}f_i = k+j$ which implies that the
  total number of hits in all scheduling rounds is $k+j+p$.


  Finally, we bound the number of faults in the scheduling rounds by case
  analysis for all cores $p_1, \ldots, p_p$.
  \begin{description}
  \item[Case 1: $p_i$ faults while any other core $p'_i (p_i \neq p'_i)$ incurs
    a hit.] Let a \defn{hit-fault} be a fault while at least one other core
    incurs a hit. The number of hit-faults $f^h$ is bounded by $p$ times the
    number of hits (which is bounded above). In summary, $f^h$ is at most
    $p(k+j+p)$ while the cost of \opt is at least $j$.
  \item[Case 2: $p_1$ faults while all other cores fault or fetch.] Let a
    \defn{fault-fault} be a a fault while all other cores are faulting or
    fetching. Consider a fault-fault $f$ by $p_i$ at timestep $t$ during the
    scheduling round of core $p_i$. No hit occurs while $f$ is fetched. In
    particular, $p_i$ incurs a fault as well, so any fault-fault that takes
    place in the scheduling round of $p_i$ can be mapped to a fault by $p_i$ in
    that round.  We map the fault that starts during $f$ from all other
    cores $p'_{i} \neq p_i$ , so each fault-fault is mapped to exactly $p$ other
    faults.

    Therefore, if there are $x_i$ faults by $p_i$ in its scheduling round, there
    will be at most $p x_i$ faults by all cores during that round. Let $x^*$
    denote the maximum values among all $x_i$'s, that is, the maximum number of
    faults a core incurs in its scheduling round. The number of fault-faults is
    at most $p(\sum\limits^p_{i = 1} x_i) \leq p^2x^*$. On the other hand, $x^*/k$ is
    a lower bound for the cost of \opt during the whole phase. This is because
    \aaa gives the maximum possible cache size to a core, and it still incurs
    $x^*$ faults.
  \end{description}
  \pparagraph{Analysis:} The cost of \opt is at least $\max\{j, x^* \}$ and the
  cost of \aaa is at most $k+j$ (from the paging round) plus $p(k+j+p)$ (from
  hit-faults) plus $p^2 x^*$ (from fault-faults). The competitive ratio of \aaa
  is therefore
  $\frac{(p+1)(k+j)+p^2(x^*+1)}{\max\{j,x^*\}} \leq 2p^2+(p+1)(k+1)$.
%
%We count the number of faults \aaa incurs at the time-steps associated with the scheduling round of processor $p_i$.
%
%Define a time-step in any of the following scheduling rounds `good' if at least one of the processors not synced with $p^*$ has hits and `bad' if all processors incur faults or at the process of fetching at the time-step. We know in the paging round all processors incur a total of at most $k+p$ fault (the total number of request in that round). Assume $p^*$ is not fetching at the beginning of the round and incurs a hit at each time-step. All other processors have been fetching and see $\tau-1$ less requests until the finish their fetching. For each fault that they incur, they see another $\tau-1$ less requests than $p^*$. So, in total, they will see $(k+p+1)(\tau-1)$ less pages than $p^*$ in the paging round. In the time-step followed by a good round, however, they see at least one more request. So, after at most $(k+p+1)(\tau-1)$ good rounds, all processors are synced.
%
%Let $q$ denote the processor whose round in \aaa has the maximum number of faults $f_q$ (the faults by all processors). So, the number of faults by the algorithm in the scheduling phases is at most $(p-1)f_q$. The cost of \opt for serving the sub-sequecnce formed by this round of the sequence of $q$ is
%
%At the end of the paging phase, $p^*$ can be ahead of any other processor by at most $k/p$ time-step; this happens when $p^*$ was not fetching at the beginning and has hits on all request while another processor just started fetching and had faults on all its requests..
\end{proof}

==> app-related.tex <==
\section{Proofs for~\secref{related}}\label{app:related}

\lruhass*

\begin{proof}
  Let each request sequence $\req_i$ be as follows:
  $\req_i = (\sigma_1^i, \ldots, \sigma_{k/p + 1}^i)^\ell$.  We set $\ell \gg
  k$. \lru faults on all $n$ requests because it keeps evicting the page that it
  will request next. In contrast, an offline algorithm \alg can delay sequences
  at no cost can serve the request sequences in order: first $\req_1$, then
  $\req_2$ and so on. The offline algorithm \alg hits on all but the cold misses
  to bring the requests to cache, for a total of $kp$ requests. Therefore,
  $\lru(\req) / \alg(\req) = \Omega(n/kp)$.
\end{proof}


==> app-shared.tex <==
\section{Proofs for~\secref{lower-shared}}\label{app:shared}

\lowershared*
\begin{proof}
  We begin with a high-level description of the sequence and proof structure and
  then fill in the details of each part of the adversarial \inp.

  \noindent \paragraph{Intuition:} We will construct an adversarial input using
  $k$ ``blue'' and $k$ ``red'' pages ($\{b_1, \ldots, b_k\}$ and
  $\{r_1, \ldots, r_k\}$, respectively).  At a high level, the input is designed
  to adapt to \alg and composed of rounds of one ``easy'' and ``hard''
  phase. Depending on the evictions of \alg, subsequent ``easy'' and ``hard''
  phases may be different from each other between rounds. Each easy and hard
  phase is comprised of $\ell$ requests. The first round is different from the
  subsequent rounds, so we will first describe the first round and how \alg and
  an offline algorithm \off serve the requests. Then we will describe all
  subsequent rounds and analyze how \alg and \off on perform on the entire \inp
  in terms of page faults and total time. The general structure of the \inp
  $\req = \{\req_1, \req_2\}$ is as follows:
 \begin{align*}
   \req_1 & = [(\text{\small First Easy
            Phase of \redp}) (\text{\small  Hard
            Phase of \redp})] \hspace*{1mm} \\
          &  [(\text{\small Subsequent Easy
            Phase of \redp}) (\text{\small  Hard Phase of \redp})]^\phi \\
   \req_2 & = [(\text{\small First Easy
            Phase of \bluep}) (\text{\small  Hard
            Phase of \bluep})]\hspace*{1mm} \\
          & [(\text{\small Subsequent Easy Phase of \bluep}) (\text{\small
             Hard Phase of \bluep})]^{\phi}
 \end{align*}

 \paragraph{Hard phases:}
  In the hard phase, \redp requests only red pages and \bluep requests only
  blue pages adversarially. The adversary constructs the \inp to so that \redp
  always requests a red page not in the cache and \bluep always requests a blue
  page not in the cache.  Since there is at least one red and blue page in the
  cache at any time during \alg's hard phase, the adversary is always guaranteed
  at least one red and blue page outside of the cache of \alg because the entire
  set of $k$ red and $k$ blue pages cannot fit in the cache during \alg's hard
  phase.

 The adversary generates the \inp such that \redp and \bluep always start and
 finish their hard phases at the same time under \alg. Furthermore, at the
 beginning of each round, there is at least one red and one blue page in \alg's
 cache.

\noindent \paragraph{First round:}
 Let $F_1, F_2$ be the first round of $\req_1, \req_2$ respectively.
 \begin{align*}
 F_1 & = \underbrace{(b_1b_2)^{\ell/2}}_{\text{First Easy
                         Phase of \redp}} (\text{\small  Hard
       Phase of \redp}) \\
 F_2 & = \underbrace{(r_1r_2)^{\ell/2}}_{\text{First Easy
                         Phase of \bluep}} (\text{\small  Hard
       Phase of \bluep})
  \end{align*}

% There is always least one page of each color in the cache at
% any time during \alg's hard phase and $k$ pages of each color, so there is always
% at least one page of each color outside of the cache.

\paragraph{\alg during the first round:}
Since the first easy phase repeats requests to the same four pages, \alg hits
on all requests in this phase after the initial cold misses and both cores
finish the first easy phase at the same time.

Therefore, both cores finish the first round at the same time under \alg with a
total of $2(\ell + 2) = \Theta(\ell)$ faults at time
$2\tau + (\ell - 2) + \tau\ell = (\tau + 1)\ell + 2\tau - 2$.

\paragraph{\off during the first round:}
We will now describe an offline algorithm \off that ``delays'' one of the cores
in the first round so that the other can use the entire cache. During the first
easy phase (wlog), \off delays \bluep by evicting the page it will request next
on each miss. That is, on the first request to $r_2$ by \bluep (after bringing
$r_1$ to the cache), \off evicts $r_1$ so that the next request to $r_1$ is a
fault.  Since \off delayed \bluep, \redp fills the cache (incurs $k-2$ cold
misses) and then hits on the rest of requests in its first hard phase. \off
delays \bluep in this way for $\ell/\tau + k - 2$ requests so that \bluep
finishes its first easy phase when \redp finishes its first hard phase.

Under \off, \redp incurs $k$ faults during its first round and \bluep incurs
$\ell/\tau + k - 2$ faults during its first easy phase.

% \redp finishes its first round at time
% $\tau k + (\ell - 2) + (\ell - k - 2) = 2\ell + (\tau - 1)k - 4$.

At the end of the first round of \redp, the first hard phase of \bluep starts
at the same time as the second easy phase for \redp. That is, the hard
phases of \bluep are aligned with the easy phases for \redp. We will describe
how to maintain this alignment throughout the rest of the \inp. At a high level,
the two cores ``switch'' for the rest of the sequence by allowing the other to
use all of the cache during the hard phases.

\noindent \paragraph{Subsequent rounds:} The adversary slightly modifies the
\defn{subsequent easy phase} depending on the state of \alg's cache at the end
of each round of hard phases. We construct each subsequent easy phase such
that it has $\ell$ requests to certain pages already in \alg's cache at the
beginning of the round, so \alg incurs only hits and \redp and \bluep begin
the next hard phase at the same time in all rounds.

\paragraph{Subsequent easy phases:}
The adversary constructs the easy phases such that the faults in each easy phase
for \off maintain the alignment and \redp ends its hard phase when \bluep ends
its easy phase (and vice versa). Each phase under \off has a \defn{partner
  phase} of the same color but opposite type (e.g. easy or hard) that starts at
the same time. More formally, the easy phases of \bluep are red and the hard
phases of \bluep are blue. The \ith easy phase of \redp is partnered with the
$(i-1)$-th hard phase of \bluep (for $i \geq 2$). Similarly, the \ith easy phase
of \bluep is partnered with the \ith hard phase of \redp.

Next, we describe how the adversary constructs the partnered phases. At the
beginning of each round $i$, there must be at least one red and one blue page in
\alg's cache. Let \rdelayp be a red page and \bdelayp be a blue page in \alg's
cache. Let \bluedelay (\reddelay) be the number of unique pages that \alg
requests in the corresponding hard phase.

Let \bluedelay (\reddelay) be the number of requests until the $(k-1)$-th distinct
blue (red) page is requested in the corresponding opposing hard phase of
\alg. If there are fewer than $k-1$ distinct pages in the corresponding hard
phase, \bluedelay or \reddelay is defined as $\ell$.

More formally, let $S_1, S_2$ denote all the rounds after the first one of
$\redp, \bluep$ respectively.
 \begin{align*}
   S_1 & =  [\underbrace{(\bdelayp \rdelayp)^{\bluedelay / 2}(\bdelayp)^{\ell -
         \bluedelay}}_{\text{Subsequent Easy Phase of \redp}} (\text{\small
          Hard Phase of \redp})]^{\phi-1} \\
   S_2 & = [\underbrace{(\rdelayp \bdelayp)^{\reddelay / 2}(\rdelayp)^{\ell -
         \reddelay}}_{\text{Subsequent Easy Phase of \bluep}} (\text{\small
                           Hard Phase of \bluep})]^{\phi-1}
 \end{align*}

\paragraph{\alg during subsequent  rounds:}
All requests in the easy phases are hits and all requests in the hard phases are
faults under \alg. Therefore, the number of faults per round under \alg is
$2\ell$.

% Each subsequent round takes total time $2(\ell + \tau\ell)$ for total time
% $2\phi(\tau + 1)\ell$.

\paragraph{\off during subsequent rounds:}

Since \off delayed the first easy phase of \bluep, it can use the initial delays
to continue delaying cores to maintain the alignment with a small cost in each
round.

\off maintains the alignment of partnered easy and hard phases by evicting
\bluep (\redp) during the easy phase whenever it incurs a fault in the partnered
hard phase. In a subsequent easy phase, the adversary constructs the \inp such
that \redp requests $(\bdelayp \rdelayp)^{\bluedelay/2}$ and \bluep requests
$(\rdelayp \bdelayp)^{\reddelay/2}$ for the first \bluedelay (or \reddelay)
requests, then all \bdelayp or \rdelayp, respectively.

Therefore, the number of faults in each subsequent round under \off is at most
$4k$. The total time of each subsequent round is also at most $2(2k\tau + 2\ell)$.

\noindent \textbf{Analysis:} We will analyze the competitive ratio in terms of
both the number of faults as well as the total time.
% Let $n$ be the number of page requests of one of the request sequences (so the
% total number of requests in the entire \inp is $2n$).

\paragraph{Page faults:}
\alg incurs $\Theta(\ell)$ faults per round, for a total of
$\Theta(\ell\phi) = \Theta(n)$ faults over the entire \inp.

\off incurs at most $$(\ell/\tau + k - 2) + k + 4k(\phi - 1)$$ faults over the entire
\inp. The total number of requests over the two request sequences is
$n = 2\phi\ell$, so $\ell = n/(2\phi)$. If we set $\ell = \sqrt{n}$, then
$\phi = \sqrt{n}/2$, and the total number of faults is at most
$$\sqrt{n}/\tau + k - 2 + k + 2k\sqrt{n} - 4k \leq \sqrt{n}/\tau + 2k\sqrt{n}
\leq 4k\sqrt{n}.$$
% \helen{should there be a factor of $\tau$ in this cr? there was
%   one in the theorem statement but it didnt show up in this analysis, so i
%  removed it. anyway i put it in a command so we can change it back if needed.}

Therefore, the competitive ratio in terms of page faults is at
least $$\frac{\Theta(n)}{4k\sqrt{n}} = \lowerfaults.$$

\paragraph{Total time:} The cost of \alg is $\Theta(\tau n)$ because it faults
on a constant fraction of the requests.

We denote the number of faults that \redp and \bluep incur under \off with
$C_1$ and $C_2$, respectively. Let $C = \max(C_1, C_2)$. The time that each core
takes is bounded by the time it takes to serve all faults and hits. That
is, $$\off(\req) \leq 2(\tau C + (n/2 - C)) = 2((\tau - 1)C + n/2).$$

From the analysis in page faults, $C \leq 4k\sqrt{n}$, so $$\off(\req) \leq
8(\tau - 1)k\sqrt{n} + n = \Theta(n)$$

Therefore, the competitive ratio in total time is at least $$\frac{\Theta(\tau
  n)}{8(\tau - 1)k\sqrt{n} + n} = \lowertt.$$
\end{proof}

\lowerall*
\begin{proof}
  We duplicate the request sequences from~\thmref{lower-shared-2}. Let the first
  half of cores $p_1, \ldots, p_{\lfloor p/2\rfloor}$ be \emph{red} and the
  second half $p_{\lfloor p/2 \rfloor + 1}, \ldots, p_p$ be \emph{blue}.  The
  lower-bound input is then just the input defined
  in~\thmref{lower-shared-2} with the sequence for \redp and \bluep copied
  roughly $p/2$ times each. That is, each core in the red group is requesting
  the same page at the same time (and vice versa for blue).
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> appA.tex <==

\begin{proof}
  We will begin with a high-level description of our lower-bound \inp
  inspired by~\cite{LopezSa12a}. The \inp \req is composed of
  $p$ disjoint request sequences that request different pages in rounds in the
  same pattern of low-demand and high-demand phases, or \defn{easy phases} and
  \defn{hard phases}, respectively.

  We define an offline algorithm \off that staggers the cores to minimize
  the number of faults. At a high level, \off partitions the cores into
  disjoint groups of (approximately) equal size depending on how much
  augmentation \lru has and incurs delay faults to stagger each group's hard
  phase.~\figref{lru-aug} (bottom) contains an example of the alignment of \off
  during \req.

  Suppose we have augmentation factor $\alpha$. That is, $\alpha \leq p-1$ is the largest integer
  such that $h \geq \frac{k}{\alpha} + 2p$.  All cores reach the hard phase at
  the same time and fault on every request under \slru as shown
  in~\figref{lru-aug} (top), while the \alg divides the $p$ cores into $\alpha$
  groups\footnote{If $p \mod \alpha \neq 0$, we can make another group
    $G_{\alpha + 1}$ with the remainder and proceed with the proof with
    $\alpha' = \alpha + 1$.}  of size $p/ \alpha$ so that the number of requests
  at any time does not exceed the size of the cache.

  More formally, the request sequence of each core $p_i$ is:
$$ \req_i = \underbrace{((\sigma^i_a \sigma^i_b)^{(\alpha -
    1)\ell/2}}_{\text{easy phase}} \underbrace{(\sigma^i_1 \cdots \sigma^i_{k/p
    + 1})^{\ell/(k/p + 1)}}_{\text{hard phase}})^\phi.$$
where $\ell, \phi$ are parameters that will be defined later.

We will define an offline algorithm \off and analyze its faults. First, \off
partitions the cores into disjoint groups $G_1, \ldots, G_\alpha$ with
$\lfloor{p/\alpha}\rfloor$ cores each.  The length (number of requests) in
each easy phase is $(\alpha - 1)\ell$. In the first round, \off
incurs delay faults during its easy phase depending on which group it is in.
Without loss of generality, let $G_1$ complete first (incur no additional faults
than initial cold misses). $G_1$ finishes its first hard phase at time
\begin{align*}
  t_1 & = \underbrace{2\tau + ((\alpha-1)\ell - 2)}_{\text{easy phase}} + \underbrace{(k/p +
        1)\tau + (\ell - k/p - 1)}_{\text{hard phase}} \\
      % & = (\alpha - 1)\ell - 2 + (k/p + 3)\tau + \ell - k/p - 1 \\
      & = \alpha\ell - k/p - 3 + (k/p + 3)\tau.
\end{align*}

We construct \off such that the next group, $G_2$, begins its hard phase at the
end of $G_1$'s hard phase. Since \off has knowledge of the future, it can choose
to evict $\sigma_a^i$ upon a request to $\sigma_b^i$ (and vice versa) exactly
enough times to line up the sequences appropriately.

The number of induced (delay) faults $m_2$ that $G_2$ incurs is as follows:
\begin{align*}
	m_2\tau + ((\alpha - 1)\ell - m_2) & = t_1 = \alpha\ell - k/p - 3 + (k/p + 3)\tau \\
 % m_2 (\tau - 1) & = \ell - k/p - 3 + (k/p + 3)\tau \\
 % m_2 & \approx \ell/\tau - k/p\tau + k/p + 3 \\
        m_2 & \approx \ell/\tau + k/p + 3.
\end{align*}

Let $H = (k/p + 1)\tau + (\ell - k/p - 1)$ be the time required to finish one
hard phase of any core.

Therefore, $G_2$ finishes its first hard phase at time $t_2 = t_1 + H$, and any
group $G_i$ finishes its first hard phase at time $t_i = t_{i-1} + H$ because
a group will only start its hard phase when all previous groups have finished
their hard phases.

For each group $G_i$ to finish at time $t_{i-1} + H$, $G_i$ needs to incur an
additional $H/\tau$ faults over group $G_{i-1}$. That is,
$$m_i = m_{i-1} + H / \tau \approx 2 + (i-1)(\ell/\tau + k/p + 1).$$

Therefore, the initial (delay) faults over all cores $M$ is
%
\begin{align*}
	M  = \sum\limits_{i=2}^\alpha m_i
	% & = \sum\limits_{i=1}^\alpha (2 + i(k/p + 1) + i\ell/\tau) \\
	% & \leq 2\alpha + \frac{\alpha(\alpha + 1)}{2} (\ell/\tau + k/p + 1) \\
	 \leq 2\alpha + \alpha^2(\ell/\tau + k/p + 1).
\end{align*}

After the first round, all the sequences are aligned and \off maintains the
alignment by incurring faults in its easy phase. Specifically, it incurs
$(\alpha-1)(k/p + 1)$ faults per core in its each subsequent easy phase. The
total number of faults per round is therefore upper bounded by
$p\alpha(k/p+1)\leq 2\alpha k$. Therefore, the total number of faults over the
entire sequence is bounded by
\begin{align*}
  \off(\req)  \leq 2\alpha k\phi + M
              \leq 2\alpha k\phi + 2\alpha + \alpha^2(\ell/\tau + k/p + 1).
\end{align*}
%
Note that the total number of requests $n = \alpha\ell\phi p$, so
$\ell = \frac{n}{\alpha \phi p}$.
If we choose $ \phi =  \sqrt{{n}/{(2kp\tau)}}$, then we will have:
$$  \off(\req) \leq  2k\alpha\sqrt{{n}/{(2kp\tau)}} + M
  % & \leq \alpha \sqrt{\frac{2kn}{p\tau}} + 2\alpha + \alpha^2\left(
  %   \frac{1}{\alpha}\sqrt{\frac{2nk}{p\tau}} + k/p + 1 \right) \\
  % & \leq \alpha\sqrt{\frac{2kn}{p\tau}} + 2\alpha +
  % \alpha\sqrt{\frac{2kn}{p\tau}} + \alpha^2 (k/p + 1) \\
              = O(\alpha\sqrt{{kn}/{(p\tau)}}). $$
   %  \end{align*}

Next, we analyze \lru. In each round, \lru faults $2p$ times during the
easy phase (2 per core) and $\ell p$ times during the hard phase ($\ell$
per core). Therefore, for the total number of faults of \lru we have
$\slru(\req) = \phi p(\ell + 2)$.

%The total number of faults of LRU
%\lru(\req) = \phi p(\ell + 2) = \Theta(n/\alpha)$.

So the competitive ratio
$\lru(\req) / \ma(\req) =
\Omega\left(\frac{1}{\alpha^2}\sqrt{\frac{np\tau}{k}}\right)$.
\end{proof}

%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "main"
%%%% End:


==> conclusion.tex <==
\section{Conclusions}\label{sec:conclusion}

%In this paper, we demonstrate 
The results in this paper demonstrate that it is much harder for online algorithms to
compete with offline algorithms in the multi-core setting than in the
single-core setting, even when the offline algorithm does not have scheduling
power. We therefore %turn to beyond-worst-case 
considered alternative analysis measures for multi-core paging via
bijective analysis and a new related measure called surjective analysis. Among other results, %Our
%main result is a separation of 
we established the advantage of \lru over a large class of online algorithms on
sequences with locality of reference.

\iffalse
% helen - i cut this out for space
In this paper, we demonstrate the limits of competitive ratio as a measure for
online multi-core paging algorithms because of the scheduling power of the
adversary. Our results indicate that it is much harder for online algorithms to
compete with offline algorithms in the multi-core setting when compared to the
single-core paging. While previous results show that LRU is not competitive, we
proved that if the cache of LRU is augmented by a factor more than $p$ (the
number of cores) then LRU becomes competitive. We complemented this result with
a lower bound that indicates augmentation by a factor of $p-1$ or less cannot
help LRU compete with \opt. These results not only draw a complete picture for
LRU with augmentation, but also have practical significance for determining the
amount that LRU's cache should be scaled in order to provide suitable guarantees
for a desired performance. Such a ``two-step approach to system design'' is well
described in \cite{Roughgarden}.

In light of these negative results, we study a weakened adversary without
scheduling power (i.e.\ $\tau = 1$). We show that \lru is still not competitive
against \opt when it does not have scheduling power, but that there exists a
competitive online algorithm that tries to match \opt 's behavior.

Finally, we initiate beyond-worst-case analysis of multi-core paging via
bijective analysis and a new related measure called surjective analysis. These
measures directly compare online algorithms against each other rather than an
offline adversary and can incorporate properties of the request sequence
space. We show that all HL conservative algorithms are strongly equivalent under
bijective analysis and that a non-lazy version of FWF is worse than \lru (or any
lazy algorithm). We separate \lru from all other HL algorithms with a
combination of surjective analysis and concave analysis, which models locality
of reference in paging.

\fi
We conclude by explaining that we are optimistic about multi-core
paging. Multi-core paging is a canonical problem in online algorithms and
motivated by computer architectures with hierarchical memory.  %. Additionally,
Practitioners have extensively studied cache-replacement policies for multiple
cores. The need for theoretical understanding of %paging with multiple
%cores 
multi-core paging
will only grow as multi-core architectures become more prevalent. The results in this paper provide a step forward towards a better understanding of %for theoretical understanding of 
multi-core paging. %this rather challenging problem.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> packages.tex <==
\iffalse
% not sure what i did but i wanted the section titles in caps so i just added
% back in packages until it worked - helen
\usepackage{hyperref}
%\usepackage{authblk}
%\usepackage{fullpage}
\usepackage{color}
\usepackage{stfloats}
\usepackage{tikz}  %TikZ central library is called.
\usetikzlibrary{automata,positioning}
\usepackage{sidecap}
\usepackage{setup}
% \usepackage[usenames,dvipsnames]{xcolor}
% \usepackage{amsmath}
% \usepackage{clrscode}
\usepackage{graphicx}
\usepackage{algpseudocode}
\usepackage[noend,lined]{algorithm2e}
% \usepackage[sho]{enumitem}
\usepackage{array}
\usepackage{colortbl}
\usepackage{todonotes}
\usepackage{verbatim}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{ifthen}
\usepackage{tikz}
\usepackage{thmtools}
\usepackage{amstext}
\usepackage{todonotes}
\usepackage{url}
\usepackage{xstring}
\usepackage[bottom]{footmisc}
\usepackage{float}
\usepackage{cases}
\usepackage[margin=2cm]{geometry}
% \usepackage{geometry}
\usepackage{times}
\usetikzlibrary{calc, fit, shapes,intersections,arrows,matrix, topaths}
\usetikzlibrary{decorations,decorations.pathreplacing,patterns, shadows}
\usepackage{thm-restate}
\usepackage{titlesec}

% \usepackage{textlater} % MAB: this package allows us to push text
                       % later in the file
% \usepackage{booktabs} % For formal tables

% \usepackage{supertech-acm}
\usepackage{enumitem} % we may want to delete this package, but I'm
% putting it in for now
\fi
\usepackage{enumitem}
\usepackage{cases}
\usepackage{amstext}
\usepackage{float}
\usepackage{xspace}
\usepackage{color}
\usepackage{setup}
\usepackage{restatable}
\usepackage{mathtools}
\usepackage{amssymb}
% \usepackage[usenames,dvipsnames]{xcolor}
% \usepackage{amsmath}
% \usepackage{clrscode}
\usepackage{graphicx}
\usepackage{tikz}  %TikZ central library is called.
\usetikzlibrary{automata,positioning}
\usetikzlibrary{calc, fit, shapes,intersections,arrows,matrix, topaths}
\usetikzlibrary{decorations,decorations.pathreplacing,patterns, shadows}
\usepackage{thm-restate}
\usepackage{microtype}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> related.tex <==
\section{Related work}\label{sec:related}

In this section, we review alternative models proposed for multi-core paging,
including a class of models for multi-core paging called fixed interleaving and
the \hass model introduced by Hassidim~\cite{Hass10}. At a high level, these
models assume the order in which the requests are served is decided by the
adversary.  In practice, however, the schedule of an algorithm is implicitly
defined through the eviction strategies~\cite{LopezSa12a,LopezSa12b}. As such,
the free-interleaving model studied in this paper is more practical.

Some of the existing works focus on minimizing the makespan of paging strategies,
while others, including this paper, are focused on minimizing the number of
faults.
% the total time (including fetch delays) that it takes to serve all requests in
% that sequence.
In the case of single-core paging, minimizing the makespan and number of faults
are equivalent as makespan is simply $\tau$ times the number of faults.
% Suppose that $f_i$ and $h_i$ are the number of faults and hits that core $p_i$
% encounters in a request sequence $R$, respectively. Then the makespan of the
% request sequence is $\max\limits_i (\tau f_i + h_i).$
For multi-core paging, however, there is no such direct relationship between makespan and
number of faults.

Feuerstein and Strejilevich de Loma~\cite{Stre98,FeuerSt02} introduced
multi-threaded paging as the problem of determining an optimal schedule in terms
of the optimal interleaved request sequence from a set of individual request
sequences from multiple cores. More precisely, given $p$ request sequences
$\req_1, \ldots, \req_p$, they study fault and makespan minimization for a
``flattened'' interleaving of all $\req_i$'s.  Our work focuses on algorithms
for page replacement rather than ordering (scheduling) of the input
sequences. As mentioned, in practice, the schedule of page requests is embedded
in the page-replacement algorithm.

Several previous works~\cite{BarveGrVi00,CaoFeLi94,KattiRa12} studied multi-core
paging in the \defn{fixed-interleaving model} (named by Katti and
Ramachandran~\cite{KattiRa12}). This model assumes each core has full knowledge of its future
request sequence where the offline algorithm has knowledge of the interleaving
of requests. The interleaving of requests among cores is the same for all paging
algorithms and potentially adversarial (for competitive analysis).  Katti and
Ramachandran~\cite{KattiRa12} gave lower bounds and a competitive algorithm for
fixed interleaving with cores that have full knowledge of their individual
request sequences.
% In this paper, we studied algorithms with no knowledge about the future
% requests sequences and under free interleaving to minimize assumptions about
% processor scheduling.
In practice, cores %in a multi-core processor
do not have any knowledge about future
requests, and do not necessarily serve requests at the same rate. Instead, they
serve requests at different rates depending on whether they need to fetch pages
to the cache.

% Knowledge models are a family of models
% which %are orthogonal to fixed and free interleaving models in the sense that they
% assume % (i.e.\ whether
% processors have partial or full information about their future requests. %)
% are orthogonal to .  Katti and Ramachandran~\cite{KattiRa12} gave lower bounds
% and a competitive algorithm for the fixed interleaving with full knowledge.
% In contrast, we investigate algorithms with no knowledge about the future of
% their request sequences under the free interleaving model.

% In addition to the indices of input sequences which define a partial ordering
% of requests, mutli-core caching involves a more fine-grained ordering define
% through a timed scheduling. We assume serving a request takes place in
% `time-units' defined as follows.  When there is a request to a page inside the
% cache, a hit takes place; we assume the time needed for a hit is 1.

% \subheading{\hass}

Hassidim~\cite{Hass10} introduced a model for multi-core paging before
free interleaving which we call the \defn{\hass model}, which allows offline
algorithms to define an explicit schedule (ordering of requests) for the online
algorithm. Given an explicit schedule, the online algorithm serves an
interleaved sequence in the same way that a single-core algorithm does. The cost
of the algorithm, measured in terms of makespan, is then compared against the
cost of an optimal offline algorithm (which potentially serves the input using
another schedule).

Both \hass and free-interleaving models include a fetching delay upon a fault,
but \hass gives offline algorithms more power by allowing them to arbitrarily
delay the start of sequences at no cost in terms of the number of faults
(Theorem 3.1 of~\cite{Hass10}). While \hass provides useful insight about
serving multiple request sequences simultaneously, it leads to overly
pessimistic results when minimizing the number of faults as %, however, because
it gives offline algorithms an unfair advantage.

Hassidim~\cite{Hass10} showed \lru is not competitive when the objective is
minimizing the makespan (the timestep at which the last request is served). We
formalize this intuition with a similar sequence to prove the same result when
the objective is to minimize the number of faults.
\newtheorem{observation}[theorem]{Observation}

% \begin{theorem}[LRU is not competitive under \hass]
\begin{restatable}{observation}{lruhass}
  \label{thm:lru-hass}
  Let \alg be an offline algorithm with cache size $k$ and assume \lru has strictly
  less than $p$-augmentation. There exists a request sequence $\req$ with $n$
  requests such that $\slru(\req) / \alg(\req) = \Omega(n / kp)$.
\end{restatable}
% \end{theorem}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> results.tex <==
% !TEX root =  main.tex


\section{Results}\seclabel{results}

In this paper, we prove the following theorem, establishing the
performance of write-optimized skip lists. 



\begin{theorem}\thmlabel{main-results}
  Consider an $N$-element write-optimized skip list running in
  external memory. Let memory-hierarchy parameters $B$ and $M$ obey
  the ``tall-cache'' assumption\footnote{This tall-cache assumption has not been optimized
  and only reflects the needs of the general proof. In practice $M = \omega(B^2)$ should be a
  good enough lower-bound.} that $M = \omega(B^6)$, let the block
  size $B$ be large enough that $\min\{B^\epsilon,B^{1-\epsilon}\} \geq \log N$,
  and let $N = \omega(M^{7/6})$.

  A skip list that performs insertions and queries achieves the
  following I/O bounds for tunable performance 
  parameter $0<\epsilon<1$:

  \begin{itemize}

  \item Insertions take
    $O\left(\frac{\log_{B^\varepsilon}N}{B^{1 - \varepsilon}}\right)$ amortized I/Os
    in expectation and w.h.p.

  \item Range queries returning $K$ elements take
    $O(\log_{B^\varepsilon}N + K/B)$ I/Os in expectation and
    w.h.p. (considering point queries as range queries with $K=1$)

  \item The structure consumes $O(N)$ space, in expectation and
    w.h.p.

  \end{itemize}

  %\mab{Simon and Tyler, as you go through the math, please
  %  figure out how much larger $N$ has to be for our guarantees to apply.
  %}
  %\simon{The condition $N = \omega(M^{4/3})$ come from the fact that the
  %cached region must only be made of shallow nodes for the analysis to hold.}
  
  %\mab{I'm impressed that $M$ doesn't need to be that much larger than $B$! We should check this very carefully to confirm.}
  
  %\simon{$\omega(B^2\log B)$ means any function $f(B)$ such that $\forall c>0, f(B) > cB^2\log B$ for $B$ big enough.}

\end{theorem}




%\mfc{do we need to list the technical conditions from theorem1 ?  Or say they are the same?}
%\begin{theorem}\thmlabel{main-inserts-deletes}
%  Under the ``tall-cache'' assumption that $M = \omega(B^2\log^4 B)$,
%  a skip list that performs insertions, deletions and queries achieves the following bounds:
%
%  \begin{itemize}
%
%  \item Insertions and deletions take
%    $O\left(\frac{\log_{B^\varepsilon}N}{B^{1 - \varepsilon}}\right)$ amortized I/Os
%     in expectation and w.h.p., and the space remains linear.
%
%%   \item Point queries take $O(\epsilon \log_B N)$ I/Os w.h.p.
%
%   \item Range queries take $O(\log_{B^\varepsilon} N + K'/B)$ I/Os
%     in expectation and w.h.p, where $K'$ is the number of elements
%     that existed at any time in the range in the last $\Theta(N)$
%     steps. Since the write-optimized skip list can be implemented
%     with flush-on-query, the amortized range-query cost is
%     $O(\log_{B^\varepsilon} N + K/B)$ I/Os in expectation and w.h.p,
%     where $K$ is the number of elements currently in the range.
%     \rob{I think it should be $K/B$ no matter the flushing policy.
%       It is for the $B^\epsilon$-tree.}
%
%  \end{itemize}
%\end{theorem}

The write-optimized skip list's guarantees (like those of
a regular skip list) are based on an adversary that gets to issue
operations arbitrarily, but does not have access to the internals of
the data structure and has no way of learning the heights of the
elements in the structure.

There are two natural design choices for node splits in a
write-optimized skip list. An element with height $h$ will trigger a
split of node at heights $0,1,\ldots,h$. These node splits can be
triggered once the element has reached the leaves (``on the way up,''
as with a B-tree or \bet) or as soon as the element enters the buffer
at height $h+1$ (``on the way down'').

Interestingly, our high-probability bounds for updates require splits
on the way down, although our expectation bounds hold in both cases.
As we describe in \secref{conclusion}, splitting on the way down may
have additional benefits, in that it may help make simpler concurrent
implementations.





% \noindent\simon{Is a list of item ok for an article?} 
% \mab{Why not turn this directly into a theorem? We can have one
%   theorem for inserts, and one for deletes, if necessary. Or maybe the
%   one with deletes. Or make the other a corollary. Bullets can
%   certainly be ok. And may look great as part of the theorem. }
 
% \noindent
% In this paper, we prove that our construction of external memory write optimized skip list achieves:
% \begin{itemize}

% \item $\log_B(N)$ \textbf{worst case} I/O complexity point queries w.h.p.
% \item $\log_B(N) + K/B$ \textbf{worst case} I/O complexity range queries w.h.p, where $K$ is the number of keys in the requested range.
% \end{itemize}
% Then, one can extend the data structure with delete operations and achieve:
% \begin{itemize}
% \item $\log_B(N)/B^{1 - \varepsilon}$ \textbf{amortized} I/O complexity insertions/deletions w.h.p.
% \item $\log_B(N)$ \textbf{worst case} I/O complexity point queries w.h.p.
% \item $\log_B(N) + K/B$ \textbf{amortized} I/O complexity range queries w.h.p.
% \end{itemize}
% It remains as an open problem whether one can implement range queries with an optimal worst case complexity.
% \simon{TODO, maybe it's not an open problem anymore...}


 
%\subsection{Related Work}

%\noindent
%Skip Lists, write optimized data structures hinted at in intro story
%line, external memory skip lists, Michael, Cindy and co. PODS paper
%with HI skip list.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> temp <==
 Every processor with multiple cores
  sharing a cache needs to implement a cache-replacement algorithm. Despite the
  widespread use of multicore systems, our theoretical understanding of caching
  algorithms in the multicore setting lags far behind our understanding of the
  single-core setting.  In this paper, we consider the free-interleaving model
  for multicore caching, where a set of cores issues online requests to a shared cache. If a
  requested page by a core $p$ is in the cache, $p$ can issue another request in
  the next timestep. Otherwise, it takes $\tau>1$ timesteps to fetch the requested page to
  the cache before $p$ can make its next request. Meanwhile, other cores can
  continue issuing requests while $p$ is fetching. Hence, a page-replacement
  policy implicitly defines a schedule that defines how requests are served at
  any timestep.

  Previous work demonstrated that the competitive ratio of a large class of
  online algorithms, including Least-Recently-Used (LRU), grows with the length
  of the input. Furthermore, even offline algorithms like Furthest-In-Future,
  the optimal algorithm in single-core caching, cannot compete in the multicore
  setting.  These negative results motivate a more in-depth comparison of multicore
  caching algorithms via alternative analysis measures. Specifically, the power
  of the adversary to adapt to online algorithms suggests the need for a direct
  comparison of online algorithms to each other.

  In this paper, we introduce cyclic analysis, a generalization of bijective
  analysis introduced by Angelopoulos and Schweitzer [JACM'13]. Cyclic analysis
  captures the advantages of bijective analysis while offering flexibility that
  makes it more useful for comparing algorithms for a variety online
  problems. In particular, we take the first steps beyond worst-case analysis
  for analysis of multicore caching algorithms.  We use cyclic analysis to establish
  relationships between multicore caching algorithms, including the advantage of LRU over all
  other multicore caching algorithms in the presence of locality of reference.

